Maximizing revenue in the presence of intermediaries

We study the mechanism design problem of selling $k$ items to unit-demand buyers with private valuations for the items. A buyer either participates directly in the auction or is represented by an intermediary, who represents a subset of buyers. Our goal is to design robust mechanisms that are independent of the demand structure (i.e. how the buyers are partitioned across intermediaries), and perform well under a wide variety of possible contracts between intermediaries and buyers. We first study the case of $k$ identical items where each buyer draws its private valuation for an item i.i.d. from a known $\lambda$-regular distribution. We construct a robust mechanism that, independent of the demand structure and under certain conditions on the contracts between intermediaries and buyers, obtains a constant factor of the revenue that the mechanism designer could obtain had she known the buyers' valuations. In other words, our mechanism's expected revenue achieves a constant factor of the optimal welfare, regardless of the demand structure. Our mechanism is a simple posted-price mechanism that sets a take-it-or-leave-it per-item price that depends on $k$ and the total number of buyers, but does not depend on the demand structure or the downstream contracts. Next we generalize our result to the case when the items are not identical. We assume that the item valuations are separable. For this case, we design a mechanism that obtains at least a constant fraction of the optimal welfare, by using a menu of posted prices. This mechanism is also independent of the demand structure, but makes a relatively stronger assumption on the contracts between intermediaries and buyers, namely that each intermediary prefers outcomes with a higher sum of utilities of the subset of buyers represented by it.

==> 02BayesianMechanisms.tex <==

\subsection{Single Aggregator Only}

In this section, we consider try to approximate the  revenue maximizing mechanism
where we have a single aggregator consisting of $n$ providers. Furthermore, we consider
the case where the aggregator-providers come from a known distribution $F$. 

\subsection{Multiple Aggregators and NonAggregators}


\begin{lemma}
Let A be any individually rational and truthful deterministic mechanism for instance I of the BMUMD.
Then the expected revenue of A, RA, is no more than the expected revenue of Myerson’s mechanism for the singleparameter instance with copies, I
copies
\end{lemma}

\ggnote{Write about why doesn't standard prophet  inequality capture the problem?}

\section{Comparison to Welfare}

One way to show that there is a mechanism is that achieves a constant fraction of
welfare. We will set a price $\pi_i$ for the aggregator. If $\pi_i$ is rejected the algorithm stops. 


Observe that for MHR distributions the corresponding function $U\circ \exp$ is monotone and increasing. 

Our main theorem is the following
\begin{theorem}[Renyi's Representation]
Let $X^{(1)} \geq \dots \geq  X^{(n)}$ be the order statistics of
a sample from distribution $F$, let $U = (1/(1 − F))^{\leftarrow}$, let $Y^{(1)} \geq Y^{(2)} \geq \dots \geq Y^{(n)}$ be the
order statistics of an independent sample of the standard exponential distribution, then

\[ \left(Y^{(n)},\dots, Y^{(1)} \right) \sim \left( \frac{E_n}{n}, \dots, \sum_{k=i}^n \frac{E_k}{k}, \dots, , \sum_{k=1}^n \frac{E_k}{k} \right)\]
 
where $E_1, . . . , E_n$ are independent and identically distributed standard exponential random variables, and 
$\left(X^{(n)}, \dots, X^{(1)} \right ) \sim \left( U \circ \exp (Y^{(n)}), \dots , U \circ \exp(Y^{(1)} \right)$. 

\end{theorem}

We will use 
\begin{lemma} [Lemma 4.3~\cite{boucheron2012concentration}]

\end{lemma}

\subsubsection*{The power of bundling}

The objective of this section is to show that {\em IC-competitive mechanisms}, mechanisms that are IC mechanisms even when advertisers where directly bidding in the platform, can obtain a revenue which is arbitrarily smaller than the optimal mechanism. Hence, the collusive behavior of the aggregator benefits the seller. The intuition behind that comes from the fact that in the presence of single bidder aiming multiple objects the seller is able to propose complex mechanisms that include different bundles for the items while such mechanisms cannot be implemented by an IC-competitive mechanism. 

To prove this assertion, Lemma~\ref{lem:welf} shows that the revenue obtained by any competitive mechanism can be arbitrarily smaller compared to the welfare. We conclude use Theroem~?? which shows the existence of a (non-competitive) mechanism which is a constant factor of the welfare.  

\begin{lemma}
The revenue maximizing IC-competitive mechanism consists of a $k+1$ price auction with reserve price $r=MR^{-1}_F(0)$.
\end{lemma}

\begin{proof}

\end{proof}

\begin{lemma}
A constant $c>0$ exists such that the revenue of the optimal IC-competive mechanism is no more that $c\;k \mathbb{E}[X^{k+1}]$.  
\end{lemma}
\begin{proof}

\end{proof}

\begin{lemma}
For any constant $c>0$, there exists a distribution $F$ and $N>0$, such that $$ \sum_{i=1}^k \mathbb{E}[X^{(i)}] > c k \mathbb{E}[X^{k+1}]$$.  
\end{lemma}
\begin{proof}
For $n\in \N$, consider the family of random variables $H_n:= \sum_{i=1}^n \frac{E_i}i $ where $E_i$ are iid standard exponential random variables. 

\begin{lemma}{
For every $n,k$ and $c>0$, there exists a $G$ convex such that 
$$\E[ \sum_{i=1}^k G(H_n-H_i)] > c k \E[G(H_n-H_k)].$$}
\end{lemma}
\begin{proof}
Indeed consider $G_j(x)=x^j$, which corresponds to the hazard rate of a Weibull distribution of parameters $(1,j+1)$. Then, we have that
\begin{align*}
    \E[ \sum_{i=1}^k G(H_n-H_i)] &= \sum_{i=1}^k \E[(H_n - H_i)^j]\\
    & = \sum_{i=1}^k \E[(H_n -H_k + H_k- H_i)^j]\\
    &> k \E[(H_n -H_k)^j]+ \sum_{i=1}^k \E[j (H_n- H_k)^{j-1} (H_k-H_i)] \\
    & = k \E[(H_n -H_k)^j]+ j\E[(H_n- H_k)^{j-1}]\underbrace{\left(\sum_{i=1}^k\E[(H_k-H_i)]\right)}_{M_1(n,k)}.
\end{align*}
The equality in the last step comes from the fact that, given the definition of $H_n$, $\{H_k-H_i\}$ and $\{H_n -H_k\}$ are independent random variables.

In the next paragraph we show that a constant $M_2(n,k)>0$ exists such that $\E[(H_n- H_k)^{j-1}] > M_2(k,n) \E[(H_n- H_k)^{j}]$. As a consequence, we get that for every $j\in \N$ we have that
$$\E[\sum_{i=1}^k G_j(H_n-H_i)] > (1+M_2(n,k)M_1(n,k) j)\; \E[G_j(H_n-H_k)],$$
which proves the theorem.

Hence, to conclude we need to show that $\E[(H_n- H_k)^{j-1}] > M_2(n,k) \E[(H_n- H_k)^{j}]$ for some $M_2(n,k)>0$. Indeed, notice that
\begin{align*}
 \E[(H_n- H_k)^{j-1}] &> \E\left[\min_{i=k,\ldots,n} E^{j-1}_i \left(\sum_{i=k+1}^n \frac 1 k\right)^{j-1}\right]\\
 &=\left(\sum_{i=k+1}^n \frac 1 k\right)^{j-1} \underbrace{\int_0^{\infty} z^{j-1} (n-k)e^{-(n-k)z}dz}_{j! R(n,k)}.
\end{align*}
Similarly,


\end{proof}

\begin{theorem}
For any constant $c>0$, there exists a distribution $F$ MHR such that welfare is at least $c$ times the revenue of the optimal competitive mechanism. Mathematically, $$ \sum_{i=1}^k \mathbb{E}[X^(i)] > c k \mathbb{E}[X^{k+1}]$$.  
\end{theorem}

\begin{proof}

\end{proof}


We will now establish a scheme where an auctioneer can sell to an aggregator
by bundling the goods to get a constant fraction of the revenue of opt. 

First we need the following inequality about exponential random variables. 

%\begin{lemma} [Lemma ]










==> 05-ExtensionLambda.tex <==
\section{Extension: $\lambda$-regular distributions}\label{sec:lambda}
This section extends the results shown in previous sections to a more general class of distributions: {\em the $\lambda$-regular distributions.}

\begin{definition}[$\lambda$-regularity]\label{def:lambda-regular}
Given $\lambda\in [0,1]$, a distribution $F$ is $\lambda$-regular if $\lambda v + \frac {1-F(v)}{f(v)}$ is non-decreasing on $v\in [\underline v, \overline v]$.
\end{definition}

Observe that for $\lambda = 0$, the condition is equivalent to the monotone hazard rate condition used in the previous sections, while for $\lambda=1$, the condition is equivalent to the Myerson regularity condition (i.e, that $\phi_F(v)$ is non-decreasing). Thus, the class of $\lambda$-regular distributions smoothly interpolates between MHR and regular distributions. In particular for $\lambda>0$, this set contains heavy-tailed distributions not contained in the set of monotone hazard rate distributions (e.g. Pareto distributions correspond to $0<\lambda<1$)\footnote{The class of $\lambda$-regular distributions have been recently applied to other mechanism design problems (see \cite{schweizer2019performance} for a treatment on the topic).}

In what follows, we provide revenue guarantees on the intermediary-proof mechanisms studied in Sections~\ref{sec:robustmechanism} and \ref{sec:ext} for $\lambda$-regular distributions when $\lambda<1$. Section~\ref{sec:discussion} discuss the challenges of our mechanisms for the regular case (i.e., when $\lambda =1$). 

We first extend Facts 1-3 for the $\lambda$-regular case.

\begin{factl}\label{fact:1l} Let $F^{(1)}$ the distribution of the first order statistic of $n$ i.i.d. random variables drawn according to $\lambda$-regular distribution $F$. Then, $F^{(1)}$ is $\lambda$-regular.
\end{factl}

\begin{factl}\label{fact:12}[\cite{schweizer2019performance}] For a random variable $v$ drawn from a $\lambda$- regular distribution $F$, we have that $\P[v\ge \E[v]]\ge (1-\lambda)^{\frac 1 \lambda}$.
\end{factl}

\begin{factl}\label{fact:13}$\P[v^{(1,s-1)} \ge \E[v^{(1,s)}]] \geq \frac {s-1}s  (1-\lambda)^{\frac 1 \lambda}$.
\end{factl}

To the best of our knowledge, \Cref{fact:1l} is not known prior to our work and we provide a full proof in the Appendix. This might be of independent interest. The proof of \Cref{fact:13} follows directly from the proof used for \Cref{cor:oneless}.
 We are now in position to state the main results for the $\lambda$-regular case. \medskip

 \subsection*{The Intermediary-Proof mechanism: homogeneous case}

This section provides a revenue guarantee for the Intermediary-Proof Mechanism $(\vx^R,\vp^R)$ of Section~\ref{sec:robustmechanism} for the homogeneous case. Remember that the Intermediary-Proof Mechanism consists on a single-item posted price where each item is sold at a price $p^R = \E[v^{(1,s)}]$ with $s=\lceil n/k \rceil$. Observe that the proof of Theorem~\ref{th:1} (which tackles the monotone hazard rate case) relies on \Cref{cor:oneless}, Lemmas~\ref{lem:1} and~\ref{lem:2}. Both lemmas are independent of the shape distribution $F$ and thus hold when $F$ is $\lambda$-regular. \Cref{cor:oneless} has to be amended which we do in \Cref{fact:13}. From this discussion, we derive the following set of results.

\begin{theorem}\label{thm:lambda-regular}
Let $(\vx^R,\vp^R)$ be the Intermediary-Proof Mechanism from Definition~\ref{def:ipm_hom}. Let $\tau = \min_{\ag \in [m]} \tau_\ag$,  then for every valuation distribution $F$ that is $\lambda$-regular, and any demand structure $(m,\pi)$ we have that
\begin{enumerate}
    \item $\mbox{Rev}(F,m,\pi;(\vx^R,\vp^R) ) \ge  \tau \frac{1}{2 }  (1-\lambda)^{\frac 1 \lambda} \left(1-\frac 1 e\right)  \mbox{Wel}(F) \ge \tau  \frac{1}{2 }   (1-\lambda)^{\frac 1 \lambda} \left(1-\frac 1 e\right)   \mbox{Rev}(F,m,\pi).$
    \item If $n/k$ is an integer number, then 
    $$ \mbox{Rev}(F,m,\pi;(\vx^R,\vp^R) ) \ge  \tau (1-\lambda)^{\frac 1 \lambda} \left(1-\frac 1 e\right)  \mbox{Wel}(F) \ge \tau (1-\lambda)^{\frac 1 \lambda} \left(1-\frac 1 e\right)  \mbox{Rev}(F,m,\pi).$$
    \item $\mbox{Rev}(F,m,\pi) \ge \tau  \frac{1}{2} (1-\lambda)^{\frac 1 \lambda}\left(1-\frac 1 e\right)\mbox{Wel}(F).$
  \end{enumerate}
\end{theorem}
In words, points 1 and 2 above say that the intermediary proof mechanism obtains a constant factor of the welfare and hence revenue when $\lambda$ is a constant less than $1$. And in point 3 we obtain that the optimal revenue is a constant factor of the welfare.
%\ganote{the last item above is independent of lambda, which cannot be -- typo?}

The second result of Section~\ref{sec:robustmechanism} provides a bound on $\tau$ for the case where each intermediary is a profit-maximizer monopolist and the valuation distribution $F$ is MHR. The following lemma generalizes Lemma~\ref{lem:dm} for the case where $F$ is $\lambda$-regular case.

\begin{lemma}\label{lem:dml}
Suppose that Intermediary $\ag$ is a monopolist and only knows the prior of the buyer's valuations. If the seller posts a price $p$ per item and Buyer $\bu\in \pi(\ag)$ has valuation $v_\bu \ge p$ then the probability that Intermediary $\ag$ would like to buy one item is at least $\left({1-\lambda}\right)^{\frac 1 \lambda}.$
\end{lemma}

The proof of Lemma~\ref{lem:dml} mimics the proof of Lemma~\ref{lem:dm}. The key difficulty is in adapting the Convex Inequality~\eqref{eq:convex}, which uses the monotonicity of the hazard rate, to our setting, in which a weaker version, the {\em generalized} hazard rate, is monotone.\footnote{A distribution $F$ is $\lambda$-regular if and only if $r_\lambda (v) = \frac1 {(1-F(v))^\lambda} \cdot  h_F(v)$ is non-decreasing on $v$ (Proposition 1, \cite{schweizer2019performance}.} The proof is deferred to the appendix.
 
We conclude this section with the following corollary from Lemma~\ref{lem:dml}.
 
\begin{corollary}
Suppose that each intermediary is behaving as a monopolist and implements a profit-maximizer mechanism. Then, the robust mechanism has a $\frac 1 {2} \left({1-\lambda}\right)^{\frac 2 \lambda}. \left(1-\frac 1 e\right)$ revenue guarantee. 
\end{corollary}

\subsection*{The Intermediary-Proof mechanism: heterogeneous case}

This section provides a revenue guarantee for the Intermediary-Proof Mechanism for Heterogeneous Items described in Section~\ref{sec:ext} (see Definition~\ref{def:het}). The proof-technique is the same as for Theorem~\ref{th:1} with minor modifications that take into account the approximation factor $(1-\lambda)^{\frac 1 \lambda}$ instead of $1/e$. The proof is deferred to the appendix.

\begin{theorem}\label{th:heter-lambda}
Consider the \heteromechanism defined in Definition~\ref{def:het} and suppose that all intermediaries are surplus-maximizers. Then for any demand structure $(m,\pi)$, the revenue generated from the mechanism is at least 
$$ \left(1- e^{-1/2  (1-\lambda)^{\frac 1 \lambda}} \right) \cdot (1 - \frac 1 e) \mbox{Wel}(F). $$
\end{theorem}

\begin{comment}

Our algorithm for the set of $\lambda$-regular distribution is the same and we will show that the essentially the same proof structure carries through. To do this, let's recall our mechanism and its subsequent proof. Essentially we price each item as a function of the order statistic of $\ceil{n}{k}$. We use the MHR property to show that each item exceeds its order statistic by a constant probability. We will show that a similar property will hold for $\lambda$-regular distribution. 

Our main proof of this section will come down to showing that given a $\lambda$-regular distribution $F$,
we will show that the distribution $F^{m}$ is also $\lambda$-regular for any $m \in \mathbb{N}$. 


\begin{itemize}
    \item Talk where it comes
    \item State Fact1'
    \item State Fact2'
    \item Conclude Fact 3'
    \item Discuss that in the previous results, MHR only appeared through Fact 3 as subroutine. Therefore, by the same logic we obtain the following results.
    \item We can also characterize $\tau$ for double mariginalization. Lemma 3' which uses the fact that a lambda regular distrubtion has a convex... 
    \item For indentical case: The same mechnaism has $f(\lambda)$ constant factor approx.
    \item For normalzier ...
    \item Formal proofs are defferen to the appendix.
\end{itemize}
\end{comment}

==> lambda-regular.tex <==
%\section{Showing Lambda regularity}

\begin{proof}[Proof of Fact 3']

Given $n$ i.i.d random variables drawn according to $F$,  the distribution of the first order statistic is given by $F^n(x)$. We show that if $F$ is $\lambda$- regular then $F^{n}$ is $\lambda$-regular. From \citet{schweizer2019performance} Proposition 1.e., this is equivalent to showing that $g_\lambda\circ F^n(x)$ is a convex function where
$g_\lambda(x) = \frac{1}{\lambda} \left( \frac{1}{(1-x)^{\lambda}} - 1 \right) $.

We first consider the case that $F$ is twice differentiable. In this situation, the previous condition turns to  $(g_\lambda \circ F^n)'' \geq 0$. 

Because, 
\begin{align*}
\frac{1}{n} (g_\lambda \circ F^n)'' &= f(x)^2\left(g_\lambda''(F^n(x)) \cdot n \cdot F^{n-1}(x)^2 +  g_\lambda'(F^n(x)) (n-1)\cdot F^{n-2}(x)  \right) \\
                           &\quad  + g_\lambda'(F^n(x)) F^{n-1}(x) \cdot f'(x),\\
                           g_\lambda'(x)  &= \frac{1}{(1-x)^{1+\lambda}},\\
                           g_\lambda''(x)  &=\frac{1+\lambda}{1-x} g_\lambda'(x),
\end{align*}
 we have that $g_\lambda \circ F^n$ is convex if and only if
 $$ g_\lambda'(F^n(x)) \cdot F^{n-2}(x) \cdot \left[f(x)^2\left( \frac{1+\lambda}{1-F^n(x)} \cdot n  \cdot F^{n}(x)  + (n-1)\right)  + F(x) \cdot f'(x) \right]\geq 0.$$
 
 Using~\cref{lem:lamb-aux}, we obtain that
 \begin{align*}
\frac{1}{n} (g_\lambda \circ F^n)''    &\ge g_\lambda'(F^n(x)) \cdot F^{n-2}(x) \cdot \left[ \frac{1+\lambda}{1-F(x)}F(x) f^2(x)  + F(x) \cdot f'(x) \right] \\
   &= F^{n-1}(x)  \cdot g_\lambda'(F^n(x))  \cdot \left[ \frac{1+\lambda}{1-F(x)}f^2(x)  +f'(x) \right] \\
   &= F^{n-1}(x)  \cdot g_\lambda'(F^n(x))  \cdot \left[ \frac{1+\lambda}{1-F(x)}f^2(x)  +f'(x) \right].
\end{align*}


To conclude the proof, notice that in the last expression, the first term is trivially positive; the second term is positive since $g_\lambda'>0$; the third term is positive because $F$ is $\lambda$-regular.\footnote{A distribution twice-differentiable $F$ is $\lambda$-regular if and only if $(1-F(x))^{-\lambda}$ is convex, which is equivalent to $\frac{1+\lambda}{1-F(x)}f^2(x)  +f'(x) \ge 0$ for every $x$.} Therefore,  $g_\lambda \circ F^n$ is convex which implies that $F^n$ is a $\lambda$-regular distribution.
\end{proof}

\begin{lemma} \label{lem:lamb-aux}
Given a real $F \in [0,1]$ and $\lambda \in [0,1]$, the following inequality holds
 \begin{equation}\label{ineq:lem8} \frac{1+\lambda}{1-F^n} n F^{n} + (n-1) \geq \frac{1+\lambda}{1-F}  F 
 \end{equation}
 for every $m \in \mathbb{N}$. 
\end{lemma}
\begin{proof}

First, we assert that it is sufficient to show Inequality~\eqref{ineq:lem8} for the case $\lambda =1$. To see this, observe that Inequality~\eqref{ineq:lem8} is equivalent to 
$$ \frac{1}{1-F^n} n F^{n} + \frac{n-1}{1+\lambda} \geq \frac{1}{1-F}  F.$$  We conclude by observing that the lowest value of the left-hand-side happens when $\lambda=1$ while the right-hand-side is independent of $\lambda$.

Next, consider the function $h(F) = \frac{ n F^{n}}{ {1-F^n}} - \frac{F}{1-F} $. From the previous paragraph, we need to show that $h(F)\geq-\frac{n-1}{2}$. To this extent, we show that $h$ is decreasing and that $\lim_{F \to 1} h(F) = -\frac{n-1}{2}$. 

To tackle that $h$ is decreasing, observe that
\begin{align*}
   h'(F) &= \frac{n^2\cdot F^{n-1}}{1-F^n}  + \frac{n^2 F^{2n-1}}{(1-F^n)^2} - \frac{1}{(1-F)} - \frac{F}{(1-F)^2} \\
        &= \frac{n^2 F^{n-1}}{(1-F^n)^2} - \frac{1}{(1-F)^2}.
        \end{align*}
Thus,
      $$ (1- F)^2 h'(F) = \frac{n^2 F^{n-1}}{(\sum_{i=0}^{n-1} F^{i})^2} - 1 .$$
      Because $F^{i} \geq F^{n-1}$ for $i\leq n-1$, we conclude that $(1 - F)^2 h'(F) \leq 0$. Therefore, $h$ is decreasing on $[0,1]$.

For the last step of the proof, observe that 
\begin{align*}
    \lim_{F \to 1} h(F) &= \lim_{F \to 1} \frac{n F^n}{1-F^n} - \frac{F}{1-F} \\
    &= \lim_{F \to 1} \frac{n F^n (1-F) - (1-F^n) \cdot F }{(1-F^n) (1-F)}  \\
    \intertext{Applying L'Hopital's rule twice, we get }
   \lim_{F \to 1} h(F)  &= \frac{n^2(n-1) - (n^2-1) \cdot n }{n(n+1) - n+1} \\
    & = -\frac{n-1}{2} .
\end{align*}
\end{proof}


\begin{theorem}
The \heteromechanism defined in Definition~\ref{def:het} obtains a revenue of at least 
$$ \left(1- e^{-1/2 (1-\lambda)^{\frac 1 \lambda}} \right) \cdot (1 - \frac 1 e) Wel[F]. $$
\end{theorem}

\begin{proof}

From~\cref{lem:buyone}, which is independent of the shape of the distribution $F$,  we know that if the valuation of at least one
buyer lies in the range $[u_{\ob-1},u_{\ob}]$, then item $\ob$ will be bought. 
Thus the probability that item $\ob$ is sold is
\begin{align*}
    \P[\text{item }\ob\; \text{is sold} ] &\geq 1- \P[\text{all values lie outside}[u_{\ob-1},u_\ob ] \\
    &= 1- (1-p_\ob)^n \\
    &\geq 1- e^{-p_\ob\cdot n}
\end{align*}

Therefore the revenue we obtain will  be at least 
\begin{align*}
   \min \sum_{\ob=1}^k r_\ob &\cdot   (1- e^{-p_\ob \cdot n})  
\end{align*}
However, there are some constraints on $p_\ob$s. We have that $0 \leq p_j \leq 1$. Further, Claim~\ref{cl:1} shows that for $ \ob \geq 1$,
$$n \cdot \sum_{t \leq j} p_t \geq  \frac{\ob}{2}(1-\lambda)^{\frac 1 \lambda}.$$    

The above system can be written as a convex program
\begin{align*}
   \max \sum_{\ob=1}^k r_\ob &\cdot    e^{-p_\ob \cdot n}  \label{prog:P1} \tag{Primal}\\
   n \cdot \left(\sum_{j=1}^s p_j \right) &\geq \frac{s}{2} (1-\lambda)^{\frac 1 \lambda} \qquad \text{ for all } 1\leq s \leq k \\
   0 \leq p_\ob &\leq 1  \qquad \qquad \qquad  \text{ for all } 1\leq \ob \leq k
\end{align*}



From~\Cref{lem:optprog},  the minimum
value is achieved when  $p_1 =\dots =p_k = \frac{1}{2n} (1-\lambda)^{\frac 1 \lambda}$. Plugging this into the objective, gives us the revenue gained is at least
\begin{align*}
    & (1 - e^{-1/2(1-\lambda)^{\frac 1 \lambda} }) \cdot \sum_{i=1}^k r_i \\
    &= (1 - e^{-1/2(1-\lambda)^{\frac 1 \lambda} }) \cdot \sum_{i=1}^k i \cdot (\eta_i - \eta_{i+1}) \cdot u_i \\
    &\geq (1 - e^{-1/2(1-\lambda)^{\frac 1 \lambda} })  \left(1-\frac{1}{e} \right) \cdot \sum_{i=1}^k  (\eta_i -\eta_{i+1}) \cdot \E[ \sum_{j=1}^{i} \ostat{j}{n} ] \\
\intertext{collapsing the sum and noting that $\eta_{k+1}=0$,}
    &= (1 - e^{-1/2(1-\lambda)^{\frac 1 \lambda} })  \left(1-\frac{1}{e} \right) 
    \cdot \sum_{i=1}^k \eta_i \cdot  \ostat{i}{n}
\end{align*}
The latter quantity is the welfare and this concludes the proof. 
\end{proof}



%We first prove a small property of the $p_j$s.
\begin{claim}\label{cl:1}
For $ \ob \geq 1$,
$$n \cdot \sum_{t \leq j} p_t \geq  \frac{\ob}{2}(1-\lambda)^{\frac 1 \lambda}.$$  
\end{claim}
\begin{proof}

Observe that when $\ob =1$, 
$$np_j =n\P[x \geq \E[\ostat{1}{n}]] \geq \P[\ostat{1}{n} \geq \E[\ostat{1}{n}]] \geq (1-\lambda)^{\frac 1 \lambda}.$$ Here the first inequality follows from union bound and the second inequality follows from~\Cref{lem:2}'.
% the claim is a (weaker) consequence of~\Cref{lem:2}.
For $\ob > 1$, 
$n \sum_{t \leq j} p_j = n \P[x \geq u_j]$. Recall that $u_j = E[\ostat{1}{\ceil{n/\ob}}]$.
We can partition the set of $n$ draws into $\ob$ sets each containing $s= \ceil{\frac{n}{\ob}}-1$ values. From~\Cref{cor:oneless}', we know that the maximum element in each partition will lie in the bucket with probability at least $\frac{1}{2}(1-\lambda)^{\frac 1 \lambda}$ (as $l \geq 2$). 
$$n \P[x \geq u_j] \ge j \cdot (s) \P[x \geq u_j] \geq j \cdot \P[\ostat{1}{s} \geq \E[\ostat{1}{s+1}] ] \geq j/2 (1-\lambda)^{\frac 1 \lambda}.$$
\end{proof}


\begin{lemma} \label{lem:optprog}
 Consider $r_1 \geq r_2 \geq \cdots \geq r_k \geq 0$,  then an optimal solution to the convex program \begin{align*}
   \max \sum_{\ob=1}^k r_\ob &\cdot    e^{-p_\ob \cdot n}  \label{prog:P1} \tag{Primal}\\
   n \cdot \left(\sum_{j=1}^s p_j \right) &\geq \frac{s}{2}  (1-\lambda)^{\frac 1 \lambda} \qquad \text{ for all } 1\leq s \leq k \\
   0 \leq p_\ob &\leq 1  \qquad\qquad \qquad  \text{ for all } 1\leq \ob \leq k
\end{align*}
 is $p_1 = p_2 = \dots =  p_k = \frac{1}{2n} (1-\lambda)^{\frac 1 \lambda}$.
\end{lemma}
\begin{proof}
Our proof-technique uses the complementary slackness results for convex duality. Given our Primal problem, we denote $\lambda_s$ as the dual variable corresponding to the first constraint and define $S_\ob = \sum_{s=\ob}^k \lambda_s$. Naturally $S_\ob \geq S_{\ob + 1}$. If we lagrangify the first constraint and find the optimal value of $p_\ob$, we get that $p_\ob = -\log(\frac{nS_\ob}{r_\ob})/n$. Substituting this value gives us the objective. The constraint $0 \leq p_\ob \leq 1$ gives us the second constraint on $S_j$. Thus we obtain the following dual.
\begin{align*}
   \min \sum_{\ob=1}^k S_\ob \left( n - \frac{1}{2}(1-\lambda)^{\frac 1 \lambda} \right)  &- S_\ob \cdot \log \left(\frac{nS_\ob}{r_\ob} \right)  \label{prog:D1} \tag{Dual}\\
    S_\ob &\geq  S_{\ob+1}  \qquad \quad \text{ for all } 1\leq \ob \leq k-1 \\
   \frac{r_\ob}{ne^n} \leq S_\ob &\leq  \frac{r_\ob} {n} \qquad  \qquad \text{ for all } 1\leq \ob \leq k.
\end{align*}

Consider the primal solution $p_\ob = \frac{1}{2n}(1-\lambda)^{\frac 1 \lambda}$ and observe that this is feasible and achieves an objective value of $\sum_{j=1}^k r_j e^{-1/2(1-\lambda)^{\frac 1 \lambda} }$.  Consider setting the dual to be $S_\ob = r_\ob \cdot e^{-1/2 (1-\lambda)^{\frac 1 \lambda}} / n$. Since $r_1 \geq \dots r_k \geq 0$, we know that this dual is feasible and has the same objective value. Since both the primal and dual are feasible and bounded,  we know that the primal solution $p_\ob$ is optimal. 
\end{proof}


%Now we can finish the proof of ~\cref{thm:heterorevenue}.
%\begin{proof}[Proof of~\cref{thm:heterorevenue}]

%From~\cref{lem:buyone}, we know that if the valuation of at least one
%buyer lies in the range $[u_{\ob-1},u_{\ob}]$, then item $\ob$ will be bought. 
%Thus the probability that item $\ob$ is sold is
%\begin{align*}
 %   \P[\text{item }\ob\; \text{is sold} ] &\geq 1- \P[\text{all values lie outside}[u_{\ob-1},u_\ob ] \\
  %  &= 1- (1-p_\ob)^n \\
   % &\geq 1- e^{-p_\ob\cdot n}
%\end{align*}

%Therefore the revenue we obtain will  be at least 
%\begin{align*}
 %  \min \sum_{\ob=1}^k r_\ob &\cdot   (1- e^{-p_\ob \cdot n})  
%\end{align*}
%However, there are some constraints on $p_\ob$s. We have that $0 \leq p_j \leq 1$. Further, for$ \ob \geq 1$,
%$$n \cdot \sum_{t \leq j} p_t \geq  \frac{\ob}{2e}.$$    

%The above system can be written as a convex program~\ref{prog:P1}. From~\Cref{lem:optprog},  the minimum
%value is achieved when  $p_1 =\dots =p_k = \frac{1}{2en}$. Plugging this into the objective, gives us the revenue gained is at least
%\begin{align*}
 %   & (1 - e^{-1/(2e)})  \cdot \sum_{i=1}^k r_i \\
  %  &= (1 - e^{-1/(2e)})  \cdot \sum_{i=1}^k i \cdot (\eta_i - \eta_{i+1}) \cdot u_i \\
   % &\geq (1 - e^{-1/(2e)})  \left(1-\frac{1}{e} \right) \cdot \sum_{i=1}^k  (\eta_i -\eta_{i+1}) % \cdot \E[ \sum_{j=1}^{i} \ostat{j}{n} ] \\
% \intertext{collapsing the sum and noting that $\eta_{k+1}=0$,}
  %  &= (1 - e^{-1/(2e)})  \left(1-\frac{1}{e} \right) 
   % \cdot \sum_{i=1}^k \eta_i \cdot  \ostat{i}{n}
%\end{align*}
%The latter quantity is the welfare and this concludes the proof. 
%\end{proof}

%\newpage

%Assume $F$ is twice differentiable, then the condition $g\circ F^m$ is a convex function is equivalent to show that 
% $$ 0 \le  (g\circ F^m)'' = g''(F^m(x))\cdot f^2(x) + g'(F(x)) \cdot f'(x) .$$

% Because $g'(y)  = \frac{1}{(1-y)^{1+\lambda}}$ and $g''(y)  =  (1+\lambda) \frac{1}{(1-y)^{2+\lambda}} =\frac{1+\lambda}{1-y} g'(y)$, we have that
% $$(g\circ F)'' = g'(F(x))\cdot \left(\frac{1+\lambda}{1-F(x)} f^2(x) +f'(x)  \right).$$





%\begin{align*}
 %   g(y) &= \frac{1}{\lambda} \left( \frac{1}{(1-y)^{\lambda}} - 1 \right) \\
 %   g'(y)  &= \frac{1}{(1-y)^{1+\lambda}}  \\
  %  g''(y)  &=  (1+\lambda) \frac{1}{(1-y)^{2+\lambda}} =\frac{1+\lambda}{1-y} g'(y)   \label{eqn:lamb1} \tag{L1} \\
% \end{align*}

%\begin{lemma}
% Given $g\circ F $ is convex for $g$ defined above, we would like to show that
% $g\circ F^m$ is also convex for any $m \in \mathbb{N}$. \apnote{This equivalent to say that that the $v^{(1,m)}$ is $\lambda$-regular when $F$ is $\lambda$-regular (see Propostion 1 \cite{schweizer2019performance}).}
% \end{lemma}
% \begin{proof}

% \begin{align*}
  %  (g\circ F)' &= g'(F(x))\cdot f(x) \\
   % (g\circ F)'' &= g''(F(x))\cdot f^2(x) + g'(F(x)) \cdot f'(x) 
    % \intertext{Applying~\Cref{eqn:lamb1} to the above, we get}
    %(g\circ F)'' &= g'(F(x))\cdot \left(\frac{1+\lambda}{1-F(x)} f^2(x) +f'(x)  \right) \geq 0 \label{eqn:lamb2} \tag{L2}
% \end{align*}
% where we use the convexity of $g\circ F$ for the last inequality. 

%To show that this is convex for $F^m(x)$, we will show that
%$(g\circ F^m)'' \geq 0$. 
%\begin{align*}
 %   (g \circ F^m)' &= g' (F^m(x)) \cdot m \cdot F^{m-1}(x) \cdot f(x) \\
  % \frac{1}{m} (g \circ F^m)'' &= g''(F^m(x)) \cdot m \cdot F^{m-1}(x)^2 \cdot f(x)^2   \\
   %                        &\quad + g'(F^m(x)) (m-1)\cdot F^{m-2}(x) \cdot f(x)^2  \\
    %                       &\quad  + g'(F^m(x)) F^{m-1}(x) \cdot f'(x) \\
 %  \intertext{Replacing the above with~\cref{eqn:lamb1}, we get}
  % &= g'(F^m(x)) \cdot F^{m-2}(x) \cdot \left[ \frac{1+\lambda}{1-F^m(x)} \cdot m  \cdot F^{m}(x) \cdot f(x)^2  + (m-1)\cdot f(x)^2  + F(x) \cdot f'(x) \right]
%   \intertext{Using~\cref{lem:lamb-aux}, we can say that }
 %  &= g'(F^m(x)) \cdot F^{m-2}(x) \cdot \left[ \frac{1+\lambda}{1-F(x)}F(x) f^2(x)  + F(x) \cdot f'(x) \right] \\
 %  &= F^{m-1}(x)  \cdot g'(F^m(x))  \cdot \left[ \frac{1+\lambda}{1-F(x)}f^2(x)  +f'(x) \right] \\
 %  &= F^{m-1}(x)  \cdot g'(F^m(x))  \cdot \left[ \frac{1+\lambda}{1-F(x)}f^2(x)  +f'(x) \right]
%\end{align*}
%Observe that the first term is always positive and the remaining is simply~\cref{eqn:lamb2} restated which we know to be positive. 
% \end{proof}



\newpage

\subsubsection{Chain of intermediaries}
\ggnote{This is speculative. We can possibly put this in the open discussions.}

\begin{conjecture}\label{con:1}
Suppose that $F$ is $\lambda$-regular, then the random variable $G(v) = \mbox{MR}_F(v)$ is also $\lambda$-regular.
\end{conjecture}
I believ the conjecture holds when $f''>0$.

A chain of intermediaries of length $r$ happens when there are $1,\ldots,r$ downstream profit-maximizer intermediaries, where intermediary one 1 buys from the seller and sells to intermediary 2 $\ldots$, and intermediary $t$ buys from intermediary $t-1$ and sells to the buyer (see \cite{balseiro2019intermediation} for more details on the model). 

\begin{lemma}
        Suppose Conejcture\ref{con:1} holds. If Intermediary $l$, has that every buyer has a chain of size $r$, we have that Buyer-Disconnectability holds with $\tau_l = \tau_\lambda^t$, where $\tau_\lambda =\left({1-\lambda}\right)^{\frac 1 \lambda}.$
\end{lemma}

\begin{proof}
The proof is by induction. Lemma~\ref{lem:2} shows the base case $t=1$.

For the inductive step, \citet{balseiro2019intermediation} shows that Intermediary $l$ behaves with Intermediary $l-1$ as a buyer whose valuation is $\mbox{MR}_{F_l}(v_l)$, where $v_l$ and $F_l$ 
 are defined inductively as $v_l= MR_{F_{l+1}}(v_{l+1})$ for $l\le t$ and $v_{t+1}=v$ (buyer's valuation). The distribution $F_l$ generates the random variable associated to $v_l$ (note that $F_{t+1}=F$). Consider a price $p$ posted by the seller and define $G = \mbox{MR}_{F_1} \circ \ldots \circ \mbox{MR}_{F_t}$, then we have that
 \begin{align*}\P [ \mbox{Buyer gets object with chain } t | v_{t+1}\ge p] &= \P[ \mbox{MR}_{F_1}(v_1)\ge p| v_{t+1}\ge p]\\
 &= \P[ \mbox{MR}_{F_1}(v_1)\ge p| \underbrace{G(v_{t+1})}_{v_1}\ge G(p)]\\
 &\ge \P[ \mbox{MR}_{F_1}(v_1)\ge p| v_1\ge p, v_1\ge G(p)] \P[v_1\ge p | v_1\ge G(p) ] \\
 & = \P[ \mbox{MR}_{F_1}(v_1)\ge p| v_1\ge p] \P[v_1\ge p | v_{t+1}\ge p ] \\
 &\ge \tau_\lambda \cdot  \P[ \underbrace{\mbox{MR}_{F_1}(v_2)}_{v_1}\ge p |v_{t+1}\ge p ]\\
 & \ge \tau_\lambda \cdot \P [ \mbox{Buyer gets object with chain } t-1 | v_{t+1}\ge p]\\
 &\ge \tau_\lambda^t.
 \end{align*}
 The second equality holds because Conjecture~\ref{con:1} implies that each $F_l$ is $\lambda$-regular, this implies that $MR_{F_l}$ is increasing, and hence, $G$ is increasing. The first inequality is due to the last of iterated probabilities. The following equality holds because $G(x)\le x$ (remember that $MR_H(x)\le x$ for every distribution $H$). The second to last equality holds from Lemma~\ref{lem:2} and the fact that $F_1$ is $\lambda$-regular (Conjecture ~\ref{con:1}). The last equality is the inductive hypothesis.   
 
 
 
 
\end{proof}
        

    
    
    
    
    
    
    %&\ge \Gamma_\lambda(  H_\lambda(\mbox{ MR}^{-1}_F(p)) - H_\lambda(p)) )\\ 
    %&\ge \Gamma_\lambda\big(\; \; \max_{p\ge 0} \; H_\lambda(\mbox{ MR}^{-1}_F(p)) - %H_\lambda(p))\big)\\
    %&= \Gamma_\lambda \big( \max_{p\ge MR_F^{-1}(0)}(H_\lambda(p) - H_\lambda(\mbox{ MR}_F(p)) \big).
    %\end{align*}
    %The first inequality is due to Lemma~\ref{lem:lamb2}. The second inequality holds because $\Gamma_\lambda$ is decreasing. The the last equality holds because MR$_F$ is increasing. 




